LIME: Less Is More for MLLM Evaluation

Multimodal Large Language Models (MLLMs) are evaluated on various benchmarks, such as image captioning, visual question answering, and reasoning. However, many of these benchmarks include overly simple or uninformative samples, complicating the effective distinction of different MLLMs' performance. Furthermore, evaluating models across numerous benchmarks incurs a significant computational burden. To address these issues, we propose LIME (Less Is More for MLLM Evaluation), a refined and efficient benchmark curated through a semi-automated pipeline. This pipeline filters out uninformative samples and eliminates answer leakage by focusing on tasks that necessitate image-based understanding. Our experiments indicate that LIME reduces the number of samples by 76% and evaluation time by 77%, while also providing a more effective means of distinguishing the capabilities of different models. Notably, we find that traditional automatic metrics, such as CIDEr, are inadequate for assessing MLLMs' captioning performance; excluding the caption task score yields a more accurate reflection of overall model performance. All code and data are available at https://github.com/kangreen0210/LIME.

==> table/model_size.tex <==
% \begin{table}[h!]%[t!]
\begin{wraptable}[12]{r}{0.5\textwidth}
% \footnotesize
% \centering
\vspace {-0.5cm}
\resizebox{0.5\columnwidth}{!}{
    \begin{tabular}{l|c|c|c|c}
    \toprule
    \textbf{Model size} & \textbf{Dataset} & \textbf{GiNi} & \textbf{stdev}\\ 
    \midrule
    
     7B& \makecell{ VB\\ OB}& \makecell{0.271 \\ 0.086} & \makecell{19.041 \\ 10.836} \\ \midrule
     8B & \makecell{ VB\\ OB} & \makecell{0.128 \\ 0.046 } & \makecell{10.685\\6.270} \\ \midrule
    13B & \makecell{ VB\\ OB} & \makecell{0.174 \\ 0.043} & \makecell{13.536 \\ 6.446}  \\ \midrule
    \bottomrule
    \end{tabular}
}
\caption{：Model size}
\label{tab：Model size}
\end{wraptable}

==> table/table2.tex <==
\begin{table}[hbt!]%[t!]
\begin{center} 
\footnotesize
\resizebox{0.99\columnwidth}{!}{
    \begin{tabular}{l|l|c|c|c|c|c|c|c|c|c|c|c}
\toprule
\textbf{Setting} & \textbf{Models} & 
\textbf{overall} & \textbf{AI2D} & \textbf{ChQA} & \textbf{COCO} & \textbf{IVQA} & \textbf{OCRBen} & \textbf{OK VQA} & \textbf{POPE} & \textbf{SciQA} & \textbf{TCaps} & \textbf{TVQA}  \\

\midrule\midrule
        & llava1.5\_7b &18.33& 24.05 & 5.25 & 79.20 & 9.08 & 2.20 & 23.43 & 32.51 & 49.00 & 65.73 & 16.50 \\
        & llava-v1.5-13b &21.03& 25.90 & 5.50 & 80.89 & 12.42 & 2.70 & 32.10 & 36.60 & 48.33 & 68.73 & 19.50 \\
        & llava-v1.6-vicuna-7b &28.48& 27.10 & 43.08 & 76.05 & 22.67 & 10.90 & 12.50 & 41.10 & 47.33 & 48.35 & 39.00 \\
        & llava-v1.6-vicuna-13b &34.19& 38.10 & 54.50 & 76.62 & 28.75 & 14.70 & 16.10 & 43.10 & 53.00 & 47.83 & 43.90 \\
        & llava-v1.6-34b &40.24& 49.60 & 64.33 & 84.25 & 42.08 & 17.10 & 10.40 & 47.00 & 64.67 & 48.25 & 51.20 \\
        & llava\_llama3 &36.88& 40.72 & 64.42 & 99.35 & 22.25 & 13.90 & 34.72 & 44.24 & 61.67 & 48.71 & 40.01 \\
        & cogvlm &44.37& 31.40 & 61.67 & 29.28 & 57.25 & 19.30 & 31.70 & 55.10 & 53.67 & 38.56 & 71.20 \\
        & deepseek-vl &35.57& 37.00 & 54.67 & 54.22 & 22.33 & 11.70 & 25.00 & 48.50 & 68.33 & 83.21 & 44.80 \\
        & idefics2 &34.72& 38.10 & 13.08 & 61.23 & 23.92 & 19.60 & 35.60 & 42.00 & 78.67 & 94.51 & 56.50 \\
        & minicpm-v-1.0 &26.47& 27.90 & 35.75 & 68.96 & 13.42 & 6.70 & 6.20 & 44.00 & 60.67 & 76.65 & 37.00 \\
        & minicpm-llama3-v-2.5 &35.50& 6.60 & 69.00 & 31.91 & 48.10 & 25.70 & 25.30 & 43.10 & 6.60 & 39.86 & 61.80 \\
        & tinny-llava-v1-hf &16.92& 22.80 & 4.50 & 63.19 & 12.17 & 1.60 & 0.90 & 37.00 & 44.67 & 58.91 & 18.70 \\
        & instructblip-vicuna-7b &18.93& 21.90 & 3.00 & 102.08 & 9.08 & 2.00 & 22.10 & 45.10 & 34.33 & 53.14 & 11.40 \\
        & internvl-v1.5 &50.68& 54.81 & 87.00 & 69.24 & 70.92 & 27.90 & 35.47 & 51.69 & 0.00 & 112.63 & 69.88 \\
        & xcomposer-4khd &49.31& 54.90 & 80.42 & 97.07 & 66.17 & 24.40 & 28.13 & 46.28 & 70.00 & 78.07 & 60.30 \\
        % & mantis-idefics & 23.60 & 5.58 & 1.10 & 11.42 & 0.40 & 9.00 & 40.63 & 45.33 & 1.68 & 2.63 \\
        \multirow{-12}{*}{\textbf{VB}} & internvl-2-8b &54.28& 60.40 & 83.75 & 42.55 & 68.25 & 32.50 & 24.20 & 49.21 & 95.67 & 25.44 & 66.10 \\
        % \multirow{-12}{*}{\textbf{VB}}& internvl-2-40b & 69.20 & 88.33 & 63.10 & 73.92 & 34.90 & 19.45 & 51.69 & 98.33 & 48.94 & 77.98 \\


\midrule\midrule
        &Llava 1.5-7b &50.29& 55.20 & 18.20 & 109.00 & 25.80 & 31.50 & 53.40 & 87.00 & 69.50 & 98.00 & 46.10 \\
        &llava-v1.5-13b &52.63& 59.40 & 18.10 & 115.40 & 29.50 & 33.60 & 58.30 & 87.10 & 72.80 & 104.00 & 48.70 \\
        &llava-v1.6-vicuna-7b &61.45& 65.30 & 55.00 & 100.00 & 37.00 & 52.40 & 44.20 & 87.60 & 70.20 & 72.00 & 64.90 \\
        &llava-v1.6-vicuna-13b &64.40& 70.40 & 62.20 & 101.90 & 41.50 & 55.00 & 46.30 & 87.50 & 73.50 & 67.30 & 67.00 \\
        &llava-v1.6-34b &66.41& 76.10 & 67.40 & 114.40 & 51.90 & 58.60 & 31.00 & 85.60 & 82.70 & 69.10 & 68.90 \\
        &llama3-llava-8b &66.09& 71.60 & 69.30 & 135.00 & 37.60 & 55.00 & 60.20 & 87.80 & 73.30 & 69.60 & 65.40 \\
        &cogvlm &68.33& 61.90 & 67.00 & 28.40 & 63.30 & 59.10 & 46.90 & 88.90 & 70.50 & 44.70 & 79.70 \\
        &deepseek-vl &60.76& 63.40 & 60.60 & 67.60 & 34.30 & 43.30 & 48.70 & 87.10 & 81.70 & 110.10 & 63.20 \\
        &idefics2 &63.89& 69.20 & 26.40 & 71.90 & 37.00 & 61.60 & 53.90 & 86.80 & 87.20 & 119.10 & 71.30 \\
        % &qwen-vl-chat & 45.90 & 60.10 & 28.80 & 1.10 & 27.00 & 3.80 & 1.40 & 62.70 & 17.10 & 61.10 \\
        &minicpm-v-1.0 &51.71& 54.20 & 43.70 & 94.30 & 24.10 & 36.30 & 26.30 & 85.10 & 76.20 & 102.60 & 55.30 \\
        &minicpm-llama3-v-2.5 &69.92& 71.70 & 72.90 & 35.50 & 56.90 & 69.40 & 52.30 & 88.00 & 53.00 & 52.90 & 75.00 \\
        &tinny-llava-v1-hf &30.86& 32.30 & 11.10 & 80.90 & 22.20 & 17.20 & 3.80 & 56.30 & 58.20 & 83.10 & 38.50 \\
        &instructblip-vicuna-7b &40.62& 34.00 & 12.50 & 141.40 & 22.90 & 25.90 & 45.20 & 85.00 & 36.40 & 74.00 & 33.20 \\
        &internvl-v1.5 &78.62& 78.90 & 83.70 & 95.80 & 72.50 & 71.40 & 60.70 & 88.90 & 94.50 & 148.10 & 79.00 \\
        &xcomposer-4khd &70.55& 34.40 & 80.60 & 134.00 & 72.80 & 66.90 & 51.90 & 87.00 & 96.00 & 111.40 & 74.30 \\
        \multirow{-12}{*}{\textbf{OB}} & internvl-2-8b&78.66& 82.25 & 82.48 & 89.77 & 70.65 & 76.50 & 52.20 & 87.90 & 97.03 & 36.70 & 77.00 \\
\bottomrule
\end{tabular}
}
\end{center}
\caption{main experiment(VB vs OB): the main experiment performance comparison between vlms-bench and origin bench.}
\label{tab:Image Content Perception}
\end{table}

==> table/table2_rank.tex <==

\begin{table}[hbt!]%[t!]
\begin{center} 
\footnotesize
\resizebox{0.99\columnwidth}{!}{
    \begin{tabular}{l|l|c|c|c|c|c|c|c|c|c|c|c}
\toprule
\textbf{Setting} & \textbf{Models} & 
\textbf{overall} & \textbf{AI2D} & \textbf{ChQA} & \textbf{COCO} & \textbf{IVQA} & \textbf{OCRBen} & \textbf{OK VQA} & \textbf{POPE} & \textbf{SciQA} & \textbf{TCaps} & \textbf{TVQA}  \\

\midrule\midrule
        & internvl-2-8b ( - ) & 54.28 & 60.40 & 83.75 & 42.55 & 68.25 & 32.50 & 24.20 & 49.21 & 95.67 & 25.44 & 66.10 \\
        & internvl-v1.5 ( - )  & 50.68 & 54.81 & 87.00 & 69.24 & 70.92 & 27.90 & 35.47 & 51.69 & 0.00 & 112.63 & 69.88 \\
        & xcomposer-4khd ( - ) & 49.31 & 54.90 & 80.42 & 97.07 & 66.17 & 24.40 & 28.13 & 46.28 & 70.00 & 78.07 & 60.30 \\
        & cogvlm (\uparrow 1) & 44.37 & 31.40 & 61.67 & 29.28 & 57.25 & 19.30 & 31.70 & 55.10 & 53.67 & 38.56 & 71.20 \\
        & llava-v1.6-34b(\uparrow 1) & 40.24 & 49.60 & 64.33 & 84.25 & 42.08 & 17.10 & 10.40 & 47.00 & 64.67 & 48.25 & 51.20 \\
        & llava\_llama3(\uparrow 1) & 36.88 & 40.72 & 64.42 & 99.35 & 22.25 & 13.90 & 34.72 & 44.24 & 61.67 & 48.71 & 40.01 \\
        & mantis-idefics & 35.85 & 35.80 & 59.00 & 61.82 & 20.50 & 14.80 & 29.07 & 44.24 & 70.00 & 103.07 & 44.51 \\
        & deepseek-vl (\uparrow 4) & 35.57 & 37.00 & 54.67 & 54.22 & 22.33 & 11.70 & 25.00 & 48.50 & 68.33 & 83.21 & 44.80 \\
        & minicpm-llama3-v-2.5(\downarrow 4) & 35.50 & 6.60 & 69.00 & 31.91 & 48.10 & 25.70 & 25.30 & 43.10 & 6.60 & 39.86 & 61.80 \\
        & idefics2 (-)& 34.72 & 38.10 & 13.08 & 61.23 & 23.92 & 19.60 & 35.60 & 42.00 & 78.67 & 94.51 & 56.50 \\
        & llava-v1.6-vicuna-13b (\downarrow 2)& 34.19 & 38.10 & 54.50 & 76.62 & 28.75 & 14.70 & 16.10 & 43.10 & 53.00 & 47.83 & 43.90 \\
        & llava-v1.6-vicuna-7b(\downarrow 1) & 28.48 & 27.10 & 43.08 & 76.05 & 22.67 & 10.90 & 12.50 & 41.10 & 47.33 & 48.35 & 39.00 \\
        & mantis-siglip & 28.29 & 27.70 & 35.33 & 68.16 & 16.25 & 4.90 & 32.43 & 45.60 & 62.67 & 81.21 & 26.34 \\
        & minicpm-v-1.0(\uparrow 1) & 26.47 & 27.90 & 35.75 & 68.96 & 13.42 & 6.70 & 6.20 & 44.00 & 60.67 & 76.65 & 37.00 \\
        & llava-v1.5-13b(\downarrow 1) & 21.03 & 25.90 & 5.50 & 80.89 & 12.42 & 2.70 & 32.10 & 36.60 & 48.33 & 68.73 & 19.50 \\
        & instructblip-vicuna-7b(\uparrow 1) & 18.93 & 21.90 & 3.00 & 102.08 & 9.08 & 2.00 & 22.10 & 45.10 & 34.33 & 53.14 & 11.40 \\
        & llava1.5\_7b(\downarrow 1) & 18.33 & 24.05 & 5.25 & 79.20 & 9.08 & 2.20 & 23.43 & 32.51 & 49.00 & 65.73 & 16.50 \\

        \multirow{-12}{*}{\textbf{VB}}& tinny-llava-v1-hf ( - ) & 16.92 & 22.80 & 4.50 & 63.19 & 12.17 & 1.60 & 0.90 & 37.00 & 44.67 & 58.91 & 18.70 \\
        
\midrule\midrule
        & internvl-2-8b & 78.66 & 82.25 & 82.48 & 89.77 & 70.65 & 76.50 & 52.20 & 87.90 & 97.03 & 36.70 & 77.00 \\
        & internvl-v1.5 & 78.62 & 78.90 & 83.70 & 95.80 & 72.50 & 71.40 & 60.70 & 88.90 & 94.50 & 148.10 & 79.00 \\
        & xcomposer-4khd & 70.55 & 34.40 & 80.60 & 134.00 & 72.80 & 66.90 & 51.90 & 87.00 & 96.00 & 111.40 & 74.30 \\
        & minicpm-llama3-v-2.5 & 69.92 & 71.70 & 72.90 & 35.50 & 56.90 & 69.40 & 52.30 & 88.00 & 53.00 & 52.90 & 75.00 \\
        & cogvlm & 68.33 & 61.90 & 67.00 & 28.40 & 63.30 & 59.10 & 46.90 & 88.90 & 70.50 & 44.70 & 79.70 \\
        & llava-v1.6-34b & 66.41 & 76.10 & 67.40 & 114.40 & 51.90 & 58.60 & 31.00 & 85.60 & 82.70 & 69.10 & 68.90 \\
        
        & llama3-llava-8b & 66.09 & 71.60 & 69.30 & 135.00 & 37.60 & 55.00 & 60.20 & 87.80 & 73.30 & 69.60 & 65.40 \\
        & llava-v1.6-vicuna-13b & 64.40 & 70.40 & 62.20 & 101.90 & 41.50 & 55.00 & 46.30 & 87.50 & 73.50 & 67.30 & 67.00 \\
        & mantis-idefics & 63.68 & 66.81 & 63.56 & 79.42 & 31.17 & 54.20 & 52.50 & 86.90 & 81.80 & 134.08 & 63.51 \\

        & idefics2 & 63.89 & 69.20 & 26.40 & 71.90 & 37.00 & 61.60 & 53.90 & 86.80 & 87.20 & 119.10 & 71.30 \\
        & llava-v1.6-vicuna-7b & 61.45 & 65.30 & 55.00 & 100.00 & 37.00 & 52.40 & 44.20 & 87.60 & 70.20 & 72.00 & 64.90 \\
        & deepseek-vl & 60.76 & 63.40 & 60.60 & 67.60 & 34.30 & 43.30 & 48.70 & 87.10 & 81.70 & 110.10 & 63.20 \\
        & mantis-siglip & 53.25 & 57.84 & 42.56 & 91.37 & 26.56 & 34.50 & 52.90 & 81.47 & 75.36 & 111.43 & 49.59 \\
        & llava-v1.5-13b & 52.63 & 59.40 & 18.10 & 115.40 & 29.50 & 33.60 & 58.30 & 87.10 & 72.80 & 104.00 & 48.70 \\
        
        & minicpm-v-1.0 & 51.71 & 54.20 & 43.70 & 94.30 & 24.10 & 36.30 & 26.30 & 85.10 & 76.20 & 102.60 & 55.30 \\
        & Llava 1.5-7b & 50.29 & 55.20 & 18.20 & 109.00 & 25.80 & 31.50 & 53.40 & 87.00 & 69.50 & 98.00 & 46.10 \\
        &instructblip-vicuna-7b & 40.62 & 34.00 & 12.50 & 141.40 & 22.90 & 25.90 & 45.20 & 85.00 & 36.40 & 74.00 & 33.20 \\
        \multirow{-12}{*}{\textbf{OB}} 
        & tinny-llava-v1-hf & 30.86 & 32.30 & 11.10 & 80.90 & 22.20 & 17.20 & 3.80 & 56.30 & 58.20 & 83.10 & 38.50 \\
\bottomrule
\end{tabular}
}
\end{center}
\caption{main experiment(VB vs OB): the main experiment performance comparison between vlms-bench and origin bench.}
\label{tab:Image Content Perception}
\end{table}

==> table/table3.tex <==
\begin{table}[hbt!]%[t!]
\begin{center} 
\footnotesize
\resizebox{0.99\columnwidth}{!}{
    \begin{tabular}{l|l|c|c|c|c|c|c|c|c|c|c}
\toprule
\textbf{Setting} & \textbf{Models} & \textbf{AI2D} & \textbf{ChQA} & \textbf{COCO} & \textbf{IVQA} & \textbf{OCRBen} & \textbf{OK VQA} & \textbf{POPE} & \textbf{SciQA} & \textbf{TCaps} & \textbf{TVQA}  \\

\midrule\midrule
   
&Llama3-8B & 23.50  & 6.40  & 2.80 & 12.90  & 4.20  & 17.40 & 32.10  & 16.40 & 5.30  & 17.90  \\ 
&Llama3-70B & 24.00  & 7.70 & 3.30 & 12.30 & 4.30  & 21.80  & 38.10 & 39.40  & 6.00  & 22.00  \\ 
&Qwen1.5-32B & 28.80  & 6.70  & 6.50  & 9.40 & 4.00  & 4.70  & 39.30  & 46.60  & 9.20 & 13.70 \\ 
&Qwen1.5-72B & 25.40  & 2.50 & 3.20 & 10.10  & 4.10 & 7.80  & 42.70 & 44.20  & 6.00 & 15.20  \\ 
&Qwen2-7B & 27.60  & 6.70  & 6.90 & 11.20  & 4.10  & 15.00 & 44.20 & 45.50  & 12.50  & 19.00  \\ 
\multirow{-6}{*}{\textbf{QVD}}&Qwen2-72B & 26.30  & 6.90 & 2.70  & 10.80 & 4.40  & 10.60  & 36.30 & 45.20  & 5.20  & 16.80 \\ 
\midrule\midrule
&Internvl-v1.5 &  54.81 & 	87.00 & 	69.24 & 	70.92 & 	27.90 & 	35.47 & 	51.69 & 	0.00 & 	112.63 & 	69.88  \\ 
&Internvl-2-8b & 60.40 & 	83.75 	& 42.55 	& 68.25 	& 32.50 & 	24.20 & 	49.21 & 	95.67 & 	25.44 	& 66.10  \\ 
&Internvl-2-40b & 69.20 & 	88.33 	& 63.10 & 	73.92 & 	34.90 & 	19.45 & 	51.69 	& 98.33 & 	48.94 	& 77.98  \\
&Llava-v1.6-7b  & 27.10 & 	43.08 & 	76.05 & 	22.67 & 	10.90 	& 12.50 	& 41.10 	& 47.33 	& 48.35 & 39.00 \\ 
&Llava-v1.6-13b & 38.10 &  	54.50 	& 76.62 & 	28.75 & 	14.70 & 	16.10 & 	43.10 & 	53.00 & 	47.83 & 	43.90  \\ 
\multirow{-6}{*}{\textbf{IQ}} &Llava-v1.6-34b & 49.60 &	64.33 &	84.25 	&42.08 &	17.10 &	10.40 &	47.00 &	64.67 &	48.25 	&51.20  \\ 
\bottomrule
\end{tabular}
}
\end{center}
\caption{Text-only with VD results: With the condition of providing only text QA information and VD information, the performance comparison between vlms-bench and origin bench. In parentheses are the scores of origin bench.}
\label{tab:Image Content Perception}
\end{table}




==> table/table_model_serises.tex <==
% \begin{table}[h!]%[t!]
\begin{wraptable}[12]{r}{0.5\textwidth}
% \footnotesize
% \centering
\vspace {-0.5cm}
\resizebox{0.5\columnwidth}{!}{
    \begin{tabular}{l|c|c|c|c}
    \toprule
    \textbf{Model series} & \textbf{Dataset} & \textbf{GiNi} & \textbf{stdev}\\ 
    \midrule
    
     InternVL-2& \makecell{ VB\\ OB}& \makecell{0.063 \\ 0.030} & \makecell{6.864 \\ 4.421} \\ \midrule
     Cambrian & \makecell{ VB\\ OB} & \makecell{0.006 \\ 0.002 } & \makecell{1.227\\0.715} \\ \midrule
    LLaVA-1.6 & \makecell{ VB\\ OB} & \makecell{0.042 \\ 0.004} & \makecell{6.730 \\ 1.418}  \\ \midrule
    \bottomrule
    \end{tabular}
}
\caption{Data statics}
\label{tab：Model series}
\end{wraptable}

==> table/textonly_OB.tex <==
\begin{table}[!h]
\centering
\centering
\footnotesize
\resizebox{0.3\columnwidth}{!}{
\begin{tabular}{l|cc}
\hline
model & AI2D&ScienceQA \\
\hline
llama3-8b &25.90 & 57.00  \\ 

llama3-70b & 35.10 & 73.70 \\ 

qwen1.5-32b & 33.60 & 60.90 \\ 

qwen1.5-72b & 28.20 & 60.89 \\ 

qwen2-7b & 28.40 & 66.34 \\ 

qwen2-72b & 30.60 & 63.81 \\ 

yi-1.5-9b-chat & 26.89 & 60.31 \\ 

yi-1.5-34b-chat & 30.60 & 65.40 \\ 

yi-1.5-34b-chat & 32.39 & 67.31 \\ 
\hline
\end{tabular}
}
\caption{Text-only}
\label{tab:text-only benchmark_scores}
\end{table}

